Constrained Phi-Equilibria

The computational study of equilibria involving constraints on players' strategies has been largely neglected. However, in real-world applications, players are usually subject to constraints ruling out the feasibility of some of their strategies, such as, e.g., safety requirements and budget caps. Computational studies on constrained versions of the Nash equilibrium have lead to some results under very stringent assumptions, while finding constrained versions of the correlated equilibrium (CE) is still unexplored. In this paper, we introduce and computationally characterize constrained Phi-equilibria -- a more general notion than constrained CEs -- in normal-form games. We show that computing such equilibria is in general computationally intractable, and also that the set of the equilibria may not be convex, providing a sharp divide with unconstrained CEs. Nevertheless, we provide a polynomial-time algorithm for computing a constrained (approximate) Phi-equilibrium maximizing a given linear function, when either the number of constraints or that of players' actions is fixed. Moreover, in the special case in which a player's constraints do not depend on other players' strategies, we show that an exact, function-maximizing equilibrium can be computed in polynomial time, while one (approximate) equilibrium can be found with an efficient decentralized no-regret learning algorithm.

==> src/Envelope.tex <==
\section{newnew proof}
Let $L(z,\lambda)=\max\limits_{i \in N,\phi \in \Phi^i} \left( U^i \phi^i z- \lambda C \phi^i z - U^i z\right)$,

Clearly if $L(z,\lambda)=0$, then $z$ is an equilibrium.

We need to show that for each local minimum of the bi-convex problem it holds $L(z,\lambda)=0$.
Formally, $\bar z, \bar \lambda$ is a local minimum if:
\begin{itemize}
	\item $\min_\lambda L(\bar z,\lambda)= L(\bar z,\bar \lambda)$
	\item $\min_z L( z,\bar \lambda)= L(\bar z,\bar \lambda)$
\end{itemize}


Let $L(z,\lambda,i,\phi^i)= \left( U^i \phi^i z- \lambda C \phi^i z - U^i z\right)$
\begin{lemma}
	if $(z,\lambda)$ is a local optimum, there exists a $i(z,\lambda),\phi(z,\lambda)\in \argmax_{i \in N,\phi \in  \Phi^i} \sum_i\left( U^i \phi^i z- \lambda_i C \phi^i z - U^i z\right)$ 
	such that $\lambda=\argmin_{\lambda'} L(z,\lambda',i(z,\lambda),\phi(z,\lambda))$ and $z=\argmin_{z'} L(z',\lambda,i(z,\lambda),\phi(z,\lambda))$
\end{lemma}

Hence, $ \lambda C \phi^{i(z,\lambda}(z,\lambda) z =0$ and $  C \phi(z,\lambda) z\le 0$  by the Optimality of $\lambda$. \ma{si dimostrano facili con le KKT e Daskin}

By the optimality of z, we have that since $\phi(z,\lambda) z$ is safe for agent $i(z,\lambda)$,
\begin{align}
&\left( U^{i(z,\lambda)} \phi(z,\lambda) z- \lambda C \phi(z,\lambda) z - U^{i(z,\lambda)}  z\right) \\
&\le  \left( U^{i(z,\lambda)} \phi(z,\lambda)\phi(z,\lambda) z- \lambda C \phi(z,\lambda) \phi(z,\lambda) z - U^{i(z,\lambda)} \phi(z,\lambda) z\right)  \\
&=  \left( U^{i(z,\lambda)} \phi(z,\lambda)\phi(z,\lambda) z- \lambda C \phi(z,\lambda) \phi(z,\lambda) z - U^{i(z,\lambda)} \phi(z,\lambda) z + \lambda C  \phi(z,\lambda) z  \right) \le 0
\end{align}
where the last inequality comes from the optimality of the deviation $ \phi(z,\lambda)$.

\section{a Polynomial-time Algorithm}

\mat{non funziona un cazzo. Con gli approximate local minima non riesco a dimostrare che è un epsilon equilibrium. il problema è che $i^*, \phi^*$ non è un subgradiente per $z^*$.}


Extend $L$ with a $\delta$-strongly convex function on $z$.
Run alternate convex optimization until we find an 

$\lambda^*\in \argmin_{\lambda} L( z^*,\lambda) $
and $z^*$ such  that $L(z^*)\le \argmin_{z} L( z,\lambda^*)+\epsilon$.


By the optimality of $\lambda^*$ we have that there exists a $i^*$ and $\phi^*$ such that $ \lambda^* C \phi^* z^* =0$ and $C \phi^* z^*\le 0$.(KKT)

Let $\bar z$ be the optimal z and $i',\phi'$ the optimal deviation in $\bar z$ that satisfies the KKT.

Then, 

\begin{align}
L(z^*,\lambda^*)& \le  \left( U^{i'} \phi' \bar z- \lambda C \phi'  \bar z - U^{i'}  \bar z\right)  +\epsilon \\
& \le \left( U^{i'} \phi' \bar z- \lambda C \phi' z^* - U^{i'}  \bar z\right)  \\
&\le 
&\le \left( U^{i'} \phi^*  z^*- \lambda C \phi^*   z^* - U^{i'}  \bar z\right) + \epsilon\\
& \le \left( U^{i'} \phi^*  z^*-  U^{i'}  \bar z\right) + \epsilon\\
& \le \left( U^{i'} \phi^*  z^*-  U^{i'}  \bar z\right) + \epsilon
\end{align}


\begin{align}
L(z^*,\lambda^*)&\le L(\bar z,\lambda^*) +\epsilon\\
&=\max_{i,\phi}\left( U^{i}  \phi \bar z- \lambda C  \phi \bar z - U^{i} \phi \bar z\right) \\
&\le  \left( U^{i^*}  \phi^* \bar z- \lambda C  \phi^* \bar z - U^{i^*}  \bar z\right)   + \epsilon+ \delta \\
&=  \left( U^{i(z,\lambda)} \phi(z,\lambda)\phi(z,\lambda) z- \lambda C \phi(z,\lambda) \phi(z,\lambda) z - U^{i(z,\lambda)} \phi(z,\lambda) z + \lambda C  \phi(z,\lambda) z  \right) \le 0
\end{align}


%\section{new Proof}
%
%Let $L(z,\lambda)=\max\limits_{\phi \in \bar \Phi} \sum_i\left( U^i \phi^i z- \lambda C \phi^i z - U^i z\right)$,
%where $\bar \Phi$ is the set of deviation in which at most 1 deviation is different from the identity matrix.
%
%Clearly if $L(z,\lambda)=\max\limits_{\phi \in \bar \Phi} \sum_i\left( U^i \phi^i z- \lambda_i C \phi^i z - U^i z\right)=0$, then $z$ is an equilibrium.
%
%We need to show that for each local minimum of the bi-convex problem it holds $L(z,\lambda)=0$.
%Formally, $\bar z, \bar \lambda$ is a local minimum if:
%\begin{itemize}
%	\item $\min_\lambda L(\bar z,\lambda)= L(\bar z,\bar \lambda)$
%	\item $\min_z L( z,\bar \lambda)= L(\bar z,\bar \lambda)$
%\end{itemize}
%
%Let $L(z,\lambda,\phi)= \sum_i\left( U^i \phi^i z- \lambda C \phi^i z - U^i z\right)$
%\begin{lemma}
%if $(z,\lambda)$ is a local optimum, there exists a $\phi(z,\lambda)\in \argmax_{\phi \in \bar \Phi} \sum_i\left( U^i \phi^i z- \lambda_i C \phi^i z - U^i z\right)$ 
%such that $\lambda=\argmin_{\lambda'} L(z,\lambda',\phi(z,\lambda))$ and $z=\argmin_{z'} L(z',\lambda,\phi(z,\lambda))$
%\end{lemma}
%
%Hence, $\sum_i \lambda C \phi^i(z,\lambda) z =0$ and $\sum_i  C \phi^i(z,\lambda) z\le 0$  by the Optimality of $\lambda$. 
%%%The second one implies that $C \phi^i(z,\lambda) z=0$ for each $i$.
%
%Hence, for each constraint c we have two possibilities: 
%\begin{itemize}
%	\item  $\sum_i \lambda_c C_c \phi^i(z,\lambda) z = 0$, implying  
%	\item $\sum_i \lambda_c C_c \phi^i(z,\lambda) z <0$ and $\lambda_i=0$. 
%\end{itemize}
%Now, let $i^*$ be the only agent such that $\phi^{i^*}(z,\lambda)\neq I$.
%
%By the optimality of z, we have that since $\phi(z,\lambda) z$ is safe it holds
%\begin{align}
% &\sum_i\left( U^i \phi^i(z,\lambda) z- \lambda_i C \phi^i(z,\lambda) z - U^i z\right) \\
% &\le  \sum_i\left( U^i \phi^i(z,\lambda)  \phi^{i^*}(z,\lambda) z- \lambda_i C \phi^i(z,\lambda)  \phi^{i^*}(z,\lambda) z - U^i  \phi^{i^*}(z,\lambda)z\right) \\
% &\le \sum_{i \neq i^*} \left( U^i  \phi^{i^*}(z,\lambda) z- \lambda_i C  \phi^{i^*}(z,\lambda) z - U^i \phi^{i^*}(z,\lambda) z\right)  +  \left( U^{i^*} \phi^{i^*}(z,\lambda) \phi^{i^*}(z,\lambda)  z- \lambda_{i^*} C \phi^{i^*}(z,\lambda) \phi^{i^*}(z,\lambda) z - U^{i^*} \phi^{i^*}(z,\lambda) z\right)\\
% &\le 0+\left( U^{i^*} \phi^{i^*}(z,\lambda) \phi^{i^*}(z,\lambda) z- \lambda_{i^*} C \phi^{i^*}(z,\lambda) \phi^{i^*}(z,\lambda)  z - U^{i^*} \phi^{i^*}(z,\lambda) z\right)\le 0 ,
% \end{align}
%where the last inequality comes from the optimality of the deviation $ \phi^{i^*}(z,\lambda)$.

==> src/KKT.tex <==
\section{Correlated with KKT}

Define $V(z):=\max\limits_\phi\psi(z,\phi)$, where $\psi(z,\phi)=\sum\limits_{i}(U^i\phi^i-U^i)z$. 
%Then write the KKT for the optimization problem $\min\limits_{z\in\Delta} V(z)$: 
%
%\[
%	\begin{cases}
%		0\in\partial V(z)-\lambda+\nu 1\\
%		z_i\ge 0\\
%		\lambda_i\ge 0\\
%		\lambda_i z_i = 0\\
%		z^\top 1 = 1
%		
%	\end{cases}
%\]
%
%And by daskin's theorem we have that:
%\[
%\partial V(z) = \text{co}\left\{\sum\limits_{i} \left(U^i\phi^i-U^i\right)\Big\vert \phi\in BR(z)\right\}
%\]
%
%where $BR(z):=\argmax\limits_{\phi\in\Phi}\psi(z,\phi)$ and it is a convex polytope.
%Thus there exists a $\tilde\phi\in\text{co} BR(z)=BR(z)$ s.t. $\partial V(z)\ni\nabla_z\psi(z,\tilde\phi) = \lambda - \nu 1$ and $z,\lambda, \nu$ are variable which satisfy the KKT system.



The dual problem reads of $\min\limits_{z\in\Delta} V(z)$ reads $\sup\limits_{\lambda\ge0, \nu\in\Reals}g(\lambda,\nu)$ where: 

\[
g(\lambda,\nu) = 
%\inf\limits_{z\in \Reals^n} \left\{V(z)-\lambda^\top z+\nu(z^\top 1-1)\right\}=
-\nu + \inf\limits_{z\in \Reals^n} \left\{V(z)-\lambda^\top z+\nu z^\top 1\right\}=
	\begin{cases}
		-\nu+\inf\limits_{z\in\Reals^n}V(z)&\text{if}\quad \lambda =\nu 1\\
		-\infty&\text{otherwise}
	\end{cases}
\]

And thus the optimal value for the dual problem is attained at $\nu=0$ and $\inf\limits_{z\in\Reals^n}V(z)=0$. 
%This follows from the fact that $V(z)$ it is convex and unconstrained and thus in the optimal $z$ we have $0=\nabla_z\psi(z,\tilde\phi)=\sum\limits_{i}(U^i\tilde\phi^i-U^i)\in\partial V(z)$ for a certain $\tilde\phi\in BR(z)$ and thus $V(z)=0$ since $V(z) = \psi(z,\tilde\phi)=\nabla_z\psi(z,\tilde\phi)^\top z$. 
The fact that $\inf_zV(z)=0$ follows from the fact that $V(z)\ge0$ and $V(0)=0$.

Thus the value is $0$ also for the primal problem, since it is convex we have $0$ duality gap.

==> src/any.tex <==
\section{Find an SCE}

Prove that 
\[ \min_\lambda \max_{z \in S}  \sum_i [U^i(z)-\lambda_i C z  - \min_{\eta_i} \max_{\phi^i} ( U^i(\phi^i z)-\eta_i C \phi^i z ) ] \ge \max_{z \in S}  \min_\lambda \sum_i [U^i(z)-\lambda_i C z - \min_{\eta_i} \max_{\phi^i} U^i(\phi^i z)-\eta_i C \phi^i z    \]
\[ = \max_{z }   \min_\lambda \sum_i [U^i(z)-\lambda_i C z - \min_{\eta_i} \max_{\phi^i} (U^i(\phi^i z)-\eta_i C \phi^i z)] = \min_\lambda \max_{z } \max_\eta  \sum_i [U^i(z)-\lambda_i C z - \max_{\phi^i} U^i(\phi^i z)-\eta_i C \phi^i z = 0 \]




We have that:
\[ \min_\lambda \max_{z \in S}  \sum_i [U^i(z)-\lambda_i C z - \max_{\phi^i} U^i(\phi^i z)-\lambda_i C \phi^i z  ] = 0\]

Then, 
\[ \max_{z \in S}  \sum_i [U^i(z) - \max_{\phi^i} U^i(\phi^i z)  ] = 0.\]
This implies that there exists an safe solution with

%
%$\sum_t \max_{\phi \in S(z_t)} U^i(\phi(z))\ge \max_{\phi \in S(\sum_t z_t)} \sum_t U^i(\phi(z_t))  $ 
%
%Find a sequence $z_t$, $\lambda_t$ such that
%
%
%
%
%z final is such that 
%$ \max_{\phi feasible} \sum_t \sum_t U^i \phi z -  U^i z  \le \max_{\phi feasible} \sum_t \sum_t U^i \phi z-\lambda_t C \phi z    -  U^i z   \le \sum_t U^i \phi_t z-\lambda_t C \phi_t z    -  U^i z  \le 0$
%
%
%
%$ \max_{\phi} \sum_t  U^i \phi z_t-\lambda_t C \phi z_t    -  U^i z_t  \le \sum_t \max_{\phi} \min_{\lambda} U^i \phi z_t-\lambda C \phi z_t    -  U^i z_t \le 0$.
%
%
%
%

%LP formulation
%
%\begin{align}
% \min &\sum_i [ U^i(z)- \lambda C(z)-  y_{i,a}]  \\
% s.t. & y_{i,a} \le U^i(a',z) - \lambda C(a',z) \forall i,a' ---> \textnormal{utility deviating on a'}. 
%\end{align}





==> src/hardnessOne.tex <==
\section{PPAD-hard find an equilibrium}

\begin{theorem}
	Given an algorithm to find a $SCE$, there exists a polynomial reduction to find a $\epsilon$-NE.
\end{theorem}

\begin{proof}
	Consider a two player game with set of action $A^1$ and $A^2$ and utilities $U^1$ and $U^2$.
	Consider a new game with three players. Player 3 has action $a_{a,a',a''}$ for each $a \in A^1$, $a',a''\in A^2$ and an action $\bar a$. Moreover, $\hat A^1=A^1+\bar a$ and $\hat A^2=A^2 + \bar a$.
	$U^1(\bar a,)=0 $, $U^2(\cdot, \bar a,\cdot)=0 $. 
	$C^3(a,a' ,a_{a,a',a''})=-1$, and  $C^3(a,a'' ,a_{a,a',a''})=1$. All the other costs of player 3 are $0$.
	
	
\end{proof}
